Topology of real algebraic curves near the non-singular tropical limit

In the 1990's, Itenberg and Haas studied the relations between combinatorial data in Viro's patchworking and the topology of the resulting non-singular real algebraic curves in the projective plane. Using recent results from Renaudineau and Shaw on real algebraic curves near the non-singular tropical limit, we continue the study of Itenberg and Haas inside any non-singular projective toric surface. We give new Haas' like criteria for patchworking non-singular real algebraic curves with prescribed number of connected components, in terms of twisted edges on a non-singular tropical curve. We then obtain several sufficient conditions for patchworking non-singular real algebraic curves with only ovals in their real part. One of these sufficient conditions does not depend on the ambient toric surface. In that case, we count the number of even and odd ovals of those curves in terms of the dual subdivision, and construct some new counter-examples to Ragsdale's conjecture.

==> Submission Arxiv Topology Real Trop Curve/fonts.tex <==
%------------------Font Definitions-------------------


%----------------MathCal---------------------------

\newcommand{\cA}{{\mathcal A}}
\newcommand{\cB}{{\mathcal B}}
\newcommand{\cC}{{\mathcal C}}
\newcommand{\cD}{{\mathcal D}}
\newcommand{\cE}{{\mathcal E}}
\newcommand{\cF}{{\mathcal F}}
\newcommand{\cG}{{\mathcal G}}
\newcommand{\cH}{{\mathcal H}}
\newcommand{\cI}{{\mathcal I}}
\newcommand{\cJ}{{\mathcal J}}
\newcommand{\cK}{{\mathcal K}}
\newcommand{\cL}{{\mathcal L}}
\newcommand{\cM}{{\mathcal M}}
\newcommand{\cN}{{\mathcal N}}
\newcommand{\cO}{{\mathcal O}}
\newcommand{\cP}{{\mathcal P}}
\newcommand{\cQ}{{\mathcal Q}}
\newcommand{\cR}{{\mathcal R}}
\newcommand{\cS}{{\mathcal S}}
\newcommand{\cT}{{\mathcal T}}
\newcommand{\cU}{{\mathcal U}}
\newcommand{\cV}{{\mathcal V}}
\newcommand{\cW}{{\mathcal W}}
\newcommand{\cX}{{\mathcal X}}
\newcommand{\cY}{{\mathcal Y}}
\newcommand{\cZ}{{\mathcal Z}}

%----------------MathFrak Capital------------------

\newcommand{\fA}{{\mathfrak A}}
\newcommand{\fB}{{\mathfrak B}}
\newcommand{\fC}{{\mathfrak C}}
\newcommand{\fD}{{\mathfrak D}}
\newcommand{\fE}{{\mathfrak E}}
\newcommand{\fF}{{\mathfrak F}}
\newcommand{\fG}{{\mathfrak G}}
\newcommand{\fH}{{\mathfrak H}}
\newcommand{\fI}{{\mathfrak I}}
\newcommand{\fJ}{{\mathfrak J}}
\newcommand{\fK}{{\mathfrak K}}
\newcommand{\fL}{{\mathfrak L}}
\newcommand{\fM}{{\mathfrak M}}
\newcommand{\fN}{{\mathfrak N}}
\newcommand{\fO}{{\mathfrak O}}
\newcommand{\fP}{{\mathfrak P}}
\newcommand{\fQ}{{\mathfrak Q}}
\newcommand{\fR}{{\mathfrak R}}
\newcommand{\fS}{{\mathfrak S}}
\newcommand{\fT}{{\mathfrak T}}
\newcommand{\fU}{{\mathfrak U}}
\newcommand{\fV}{{\mathfrak V}}
\newcommand{\fW}{{\mathfrak W}}
\newcommand{\fX}{{\mathfrak X}}
\newcommand{\fY}{{\mathfrak Y}}
\newcommand{\fZ}{{\mathfrak Z}}


%----------------MathFrak Lower Case---------------


\newcommand{\fa}{{\mathfrak a}}
\newcommand{\fb}{{\mathfrak b}}
\newcommand{\fc}{{\mathfrak c}}
\newcommand{\fd}{{\mathfrak d}}
\newcommand{\fe}{{\mathfrak e}}
\newcommand{\ff}{{\mathfrak f}}
\newcommand{\fg}{{\mathfrak g}}
\newcommand{\fh}{{\mathfrak h}}
\newcommand{\fli}{{\mathfrak i}}
\newcommand{\fj}{{\mathfrak j}}
\newcommand{\fk}{{\mathfrak k}}
\newcommand{\fl}{{\mathfrak l}}
\newcommand{\fm}{{\mathfrak m}}
\newcommand{\fn}{{\mathfrak n}}
\newcommand{\fo}{{\mathfrak o}}
\newcommand{\fp}{{\mathfrak p}}
\newcommand{\fq}{{\mathfrak q}}
\newcommand{\fr}{{\mathfrak r}}
\newcommand{\fs}{{\mathfrak s}}
\newcommand{\ft}{{\mathfrak t}}
\newcommand{\fu}{{\mathfrak u}}
\newcommand{\fv}{{\mathfrak v}}
\newcommand{\fw}{{\mathfrak w}}
\newcommand{\fx}{{\mathfrak x}}
\newcommand{\fy}{{\mathfrak y}}
\newcommand{\fz}{{\mathfrak z}}


%----------------MathBB----------------------------

\newcommand{\A}{{\mathbb A}}
\newcommand{\G}{{\mathbb G}}
\newcommand{\C}{{\mathbb C}}
\newcommand{\R}{{\mathbb R}}
\newcommand{\pp}{\mathbb{P}}
\newcommand{\Q}{{\mathbb Q}}
\newcommand{\N}{{\mathbb N}}
\newcommand{\Z}{{\mathbb Z}}
\newcommand{\Qp}{{\mathbb Q}_p}
\newcommand{\K}{{\mathbb K}}
\newcommand{\F}{{\mathbb F}}
\renewcommand{\T}{{\mathbb T}}
%\newcommand{\sph}{{\mathbb S}}

%----------------MathBF Lower Case-----------------

\newcommand{\ba}{{\mathbf a}}
\newcommand{\bb}{{\mathbf b}}
\newcommand{\bc}{{\mathbf c}}
\newcommand{\bd}{{\mathbf d}}
\newcommand{\bu}{{\mathbf u}}
\newcommand{\bx}{{\mathbf x}}
\newcommand{\by}{{\mathbf y}}

%----------------MathBF Greek ---------------------

\newcommand{\bmu}{{\boldsymbol \mu}}
\newcommand{\bnu}{{\boldsymbol \nu}}

%----------------MathBF + Cal ---------------------

\newcommand{\bcE}{{\boldsymbol \cE}}




==> Submission Arxiv Topology Real Trop Curve/operators.tex <==
\usepackage{mathrsfs}
%--------------------- Usefol Operators ------------------

\newcommand{\dotcup}{\ensuremath{\mathaccent\cdot\cup}}
\newcommand{\Fr}[1]{\ensuremath{\C \langle z_1,\ldots,z_{#1}\rangle}} % Free Algebra on prescribed number of variables


%------------- Derivatives ----------------------

\newcommand{\pd}[2]
{\dfrac{\partial #1}{\partial #2}}
\newcommand{\pda}[1]{\pd{#1}{a}}
\newcommand{\pdb}[1]{\pd{#1}{b}}
\newcommand{\mpd}[3]{\dfrac{\partial^{#3} #1}{\partial #2^{#3}}}

%------------- Categories + AG ------------------

\newcommand{\Mat}{\operatorname{Mat}}
\newcommand{\conv}{\operatorname{conv}}
\newcommand{\Int}{\operatorname{int}}
\newcommand{\Nil}{\operatorname{Nil}}
\newcommand{\Id}{\operatorname{I}}
\newcommand{\Sym}{\operatorname{Sym}}
\newcommand{\coker}{\operatorname{coker}}
\newcommand{\coim}{\operatorname{coim}}
\newcommand{\im}{\operatorname{im}}
\newcommand{\ii}{\operatorname{i}}
\newcommand{\Ima}{\operatorname{Im}}
\newcommand{\Rea}{\operatorname{Re}}
\newcommand{\Hom}{\operatorname{Hom}} %External Hom
\newcommand{\iHom}{\operatorname{\underline{Hom}}} %Internal Hom
\newcommand{\shHom}{\operatorname{{\mathscr Hom}}} %Sheaf Hom
\newcommand{\cten}{\widehat{\otimes}} %Completed Tensor Product
\newcommand{\ctenp}{\widehat{\otimes}_{\pi}} %Completed Projective Tensor product
\newcommand{\cteni}{\widehat{\otimes}_{i}} %Completed Inductive Tensor product
\newcommand{\Spec}{\operatorname{Spec}}
\newcommand{\Sper}{\operatorname{Sper}}
\newcommand{\Supp}{\operatorname{Supp}}
\newcommand{\Proj}{\operatorname{Proj}}
\newcommand{\ann}{\operatorname{Ann}} %Annihilator
\newcommand{\reg}{\operatorname{reg}} %Castelnuovo-Mumford regularity
\newcommand{\rank}{\operatorname{rank}} %rank of a free module
\newcommand{\Ass}{\operatorname{Ass}} %Associated primes
\newcommand{\red}{\operatorname{red}}
\newcommand{\rered}{\operatorname{rered}}
\newcommand{\Gr}{\mathbb{G}}
\newcommand{\codim}{\operatorname{codim}}
\newcommand{\gr}{\operatorname{gr}}
\newcommand{\depth}{\operatorname{depth}}
\newcommand{\grade}{\operatorname{grade}}
\newcommand{\pdim}{\operatorname{pd}}
\newcommand{\JH}{\operatorname{JH}}
\newcommand{\End}{\operatorname{End}}
\newcommand{\rep}{\text{\bf Rep}}
\newcommand{\Ext}{\operatorname{Ext}} %Global Ext
\newcommand{\shExt}{\operatorname{{\mathscr Ext}}} %Sheaf Ext
\newcommand{\Tor}{\operatorname{Tor}} %Global Tor
\newcommand{\shTor}{\operatorname{{\mathscr Tor}}} %Sheaf Tor
% Category of ...
\newcommand{\Born}{{\mathscr Born }} %Bornological Spaces
\newcommand{\Set}{{\mathscr Set }} %Sets
\newcommand{\Ab}{{\mathscr Ab }} %Abelian Groups
\newcommand{\Aff}{{\mathscr Aff }} %Affine Schemes
\newcommand{\Sch}{{\mathscr Sch }} %Schemes
\newcommand{\Grp}{{\mathscr Grp }} %Groups
\newcommand{\Vect}{{\mathscr Vect }} %Vector Spaces
\newcommand{\Mod}[1]{#1-{\mathscr Mod }} %Modules over a ring
\newcommand{\Top}{{\mathscr Top }} %Topological Spaces
\newcommand{\CTop}{{\mathscr Ctop }} %Compact Topological Spaces
\newcommand{\Ban}{{\mathscr Ban }} %Benach Spaces
\newcommand{\LCS}{{\mathscr LCS }} %Locally Convex Spaces
\newcommand{\Frch}{{\mathscr Frch }} %Frechet Spaces
\newcommand{\Sh}[1]{{\mathscr Sh }(#1)} %Sheaves on a space
\newcommand{\diff}{\operatorname{d}}
\newcommand{\T}{\operatorname{T}}


%------------- Lie Groups and Algebras ----------

\newcommand{\GL}{\operatorname{{\mathbf GL}}}
\newcommand{\gl}{\operatorname{gl}}
\newcommand{\Quot}{\operatorname{Quot}}

%------------- Operators -------------------------

\newcommand{\tr}{\operatorname{tr}}
\newcommand{\HS}{{\mathcal HS}} % Hilbert-Schmidt
\newcommand{\TC}{{\mathcal TC}} %Trace Class
\newcommand{\dirint}{\int^{\oplus}}
\newcommand{\mvec}{\operatorname{vec}} % matrix to vector
\newcommand{\HP}{\operatorname{HP}} % Hilbert Polynomial
\newcommand{\Sp}{\operatorname{Sp}} %Spectrum
\newcommand{\adj}{\operatorname{adj}} %adjugate matrix
\newcommand{\diag}{\operatorname{diag}}

%---------------Topology-----------------------
\newcommand{\lk}{\operatorname{lk}} % Linking number
\newcommand{\Ho}{\operatorname{H}} %(co-)homology

